Validation & Testing of the CROBAR 3D Coronal Reconstruction Method with a MURaM simulation

I report on validation and testing of a novel 3D reconstruction method than can obtain coronal plasma properties from a single snapshot perspective. I first reported on the method in 2021, and I have since named it the Coronal Reconstruction Onto B-Aligned Regions, or 'CROBAR', method. The testing was carried out with a cube from a MURaM 3D MHD simulation, which affords a coronal-like 'ground truth' against which the reconstruction method can be applied and compared. I find that the method does quite well, recovering the 'coronal veil'-like features recently reported from the MURaM simulations, and allaying concerns that these features would thwart recovery of valid 3D coronal structure from a limited number of perspectives. I also find that a second perspective at between $\sim 45$ and 90 degrees, does significantly improve the reconstructions. Two distinct channels with Soft X-Ray like temperature response (peaking above 5 MK) would suffice for CROBAR's optically thin observables; barring that, a suite of AIA-like EUV passbands, with good coverage of the 3-8 MK temperature range.

==> aastex_journals.tex <==
%AASTEX journal commands
%Copied from version 5.2 (2005) by D. C. Jacobs 2008

\let\jnlatstyle=\rmfamily
\def\refatjnl#1{{\jnlatstyle#1}}%
\newcommand\aj{\refatjnl{AJ}}%
          % Astronomical Journal
\newcommand\actaa{\refatjnl{Acta Astron.}}%
  % Acta Astronomica
\newcommand\araa{\refatjnl{ARA\&A}}%
          % Annual Review of Astron and Astrophys
\newcommand\apj{\refatjnl{ApJ}}%
          % Astrophysical Journal
\newcommand\apjl{\refatjnl{ApJ}}%
          % Astrophysical Journal, Letters
\newcommand\apjs{\refatjnl{ApJS}}%
          % Astrophysical Journal, Supplement
\newcommand\ao{\refatjnl{Appl.~Opt.}}%
          % Applied Optics
\newcommand\apss{\refatjnl{Ap\&SS}}%
          % Astrophysics and Space Science
\newcommand\aap{\refatjnl{A\&A}}%
          % Astronomy and Astrophysics
\newcommand\aapr{\refatjnl{A\&A~Rev.}}%
          % Astronomy and Astrophysics Reviews
\newcommand\aaps{\refatjnl{A\&AS}}%
          % Astronomy and Astrophysics, Supplement
\newcommand\azh{\refatjnl{AZh}}%
          % Astronomicheskii Zhurnal
\newcommand\baas{\refatjnl{BAAS}}%
          % Bulletin of the AAS
\newcommand\caa{\refatjnl{Chinese Astron. Astrophys.}}%
  % Chinese Astronomy and Astrophysics
\newcommand\cjaa{\refatjnl{Chinese J. Astron. Astrophys.}}%
  % Chinese Journal of Astronomy and Astrophysics
\newcommand\icarus{\refatjnl{Icarus}}%
  % Icarus
\newcommand\jcap{\refatjnl{J. Cosmology Astropart. Phys.}}%
  % Journal of Cosmology and Astroparticle Physics
\newcommand\jrasc{\refatjnl{JRASC}}%
          % Journal of the RAS of Canada
\newcommand\memras{\refatjnl{MmRAS}}%
          % Memoirs of the RAS
\newcommand\mnras{\refatjnl{MNRAS}}%
          % Monthly Notices of the RAS
\newcommand\na{\refatjnl{New A}}%
  % New Astronomy
\newcommand\nar{\refatjnl{New A Rev.}}%
  % New Astronomy Review
\newcommand\pra{\refatjnl{Phys.~Rev.~A}}%
          % Physical Review A: General Physics
\newcommand\prb{\refatjnl{Phys.~Rev.~B}}%
          % Physical Review B: Solid State
\newcommand\prc{\refatjnl{Phys.~Rev.~C}}%
          % Physical Review C
\newcommand\prd{\refatjnl{Phys.~Rev.~D}}%
          % Physical Review D
\newcommand\pre{\refatjnl{Phys.~Rev.~E}}%
          % Physical Review E
\newcommand\prl{\refatjnl{Phys.~Rev.~Lett.}}%
          % Physical Review Letters
\newcommand\pasa{\refatjnl{PASA}}%
  % Publications of the Astron. Soc. of Australia
\newcommand\pasp{\refatjnl{PASP}}%
          % Publications of the ASP
\newcommand\pasj{\refatjnl{PASJ}}%
          % Publications of the ASJ
\newcommand\qjras{\refatjnl{QJRAS}}%
          % Quarterly Journal of the RAS
\newcommand\rmxaa{\refatjnl{Rev. Mexicana Astron. Astrofis.}}%
  % Revista Mexicana de Astronomia y Astrofisica
\newcommand\skytel{\refatjnl{S\&T}}%
          % Sky and Telescope
\newcommand\solphys{\refatjnl{Sol.~Phys.}}%
          % Solar Physics
\newcommand\sovast{\refatjnl{Soviet~Ast.}}%
          % Soviet Astronomy
\newcommand\ssr{\refatjnl{Space~Sci.~Rev.}}%
          % Space Science Reviews
\newcommand\zap{\refatjnl{ZAp}}%
          % Zeitschrift fuer Astrophysik
\newcommand\nat{\refatjnl{Nature}}%
          % Nature
\newcommand\iaucirc{\refatjnl{IAU~Circ.}}%
          % IAU Cirulars
\newcommand\aplett{\refatjnl{Astrophys.~Lett.}}%
          % Astrophysics Letters and Communications
\newcommand\apspr{\refatjnl{Astrophys.~Space~Phys.~Res.}}%
          % Astrophysics Space Physics Research
\newcommand\bain{\refatjnl{Bull.~Astron.~Inst.~Netherlands}}%
          % Bulletin Astronomical Institute of the Netherlands
\newcommand\fcp{\refatjnl{Fund.~Cosmic~Phys.}}%
          % Fundamental Cosmic Physics
\newcommand\gca{\refatjnl{Geochim.~Cosmochim.~Acta}}%
          % Geochimica Cosmochimica Acta
\newcommand\grl{\refatjnl{Geophys.~Res.~Lett.}}%
          % Geophysics Research Letters
\newcommand\jcp{\refatjnl{J.~Chem.~Phys.}}%
          % Journal of Chemical Physics
\newcommand\jgr{\refatjnl{J.~Geophys.~Res.}}%
          % Journal of Geophysical Research
\newcommand\jqsrt{\refatjnl{J.~Quant.~Spec.~Radiat.~Transf.}}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\newcommand\memsai{\refatjnl{Mem.~Soc.~Astron.~Italiana}}%
          % Mem. Societa Astronomica Italiana
\newcommand\nphysa{\refatjnl{Nucl.~Phys.~A}}%
          % Nuclear Physics A
\newcommand\physrep{\refatjnl{Phys.~Rep.}}%
          % Physics Reports
\newcommand\physscr{\refatjnl{Phys.~Scr}}%
          % Physica Scripta
\newcommand\planss{\refatjnl{Planet.~Space~Sci.}}%
          % Planetary Space Science
\newcommand\procspie{\refatjnl{Proc.~SPIE}}%
          % Proceedings of the SPIE
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao

